Sparse VideoGen2: Accelerate Video Generation with Sparse Attention via Semantic-Aware Permutation

Diffusion Transformers (DiTs) are essential for video generation but suffer from significant latency due to the quadratic complexity of attention. By computing only critical tokens, sparse attention reduces computational costs and offers a promising acceleration approach. However, we identify that existing methods fail to approach optimal generation quality under the same computation budget for two reasons: (1) Inaccurate critical token identification: current methods cluster tokens based on position rather than semantics, leading to imprecise aggregated representations. (2) Excessive computation waste: critical tokens are scattered among non-critical ones, leading to wasted computation on GPUs, which are optimized for processing contiguous tokens. In this paper, we propose SVG2, a training-free framework that maximizes identification accuracy and minimizes computation waste, achieving a Pareto frontier trade-off between generation quality and efficiency. The core of SVG2 is semantic-aware permutation, which clusters and reorders tokens based on semantic similarity using k-means. This approach ensures both a precise cluster representation, improving identification accuracy, and a densified layout of critical tokens, enabling efficient computation without padding. Additionally, SVG2 integrates top-p dynamic budget control and customized kernel implementations, achieving up to 2.30x and 1.89x speedup while maintaining a PSNR of up to 30 and 26 on HunyuanVideo and Wan 2.1, respectively. Our code is open-sourced at \href{https://github.com/svg-project/Sparse-VideoGen}{https://github.com/svg-project/Sparse-VideoGen}.

==> algorithms/weighted_softmax_topp.tex <==
\begin{figure}[t]
    \centering
      
    \begin{minipage}{0.42\textwidth}
    
    \begin{algorithm}[H]
        \caption{Top-p Centroid Selection}
        \lblalg{attention_mask_generation}
        \definecolor{codeblue}{rgb}{0.25,0.65,0.5}
        \definecolor{codeblue2}{rgb}{0,0,1}
        \lstset{
          backgroundcolor=\color{white},
          basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
          columns=fixed,
          breaklines=true,
          captionpos=b,
          commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
          keywordstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue2},
        }
        \begin{lstlisting}[language=python]
        # C: [m, d], D: [n, d] - centroids
        # p - probability (default = 0.9)
        # Compute score matrix
        A = torch.matmul(C,  D.T)  # [m, n]
        
        # Weighted softmax scores
        P = weighted_softmax(A)  # [m, n]
        
        # Select top-p indices
        indices = top_p(P, p)  # [m, b]
        \end{lstlisting}
    \end{algorithm}
    
    \end{minipage}
    \hfill
    \begin{minipage}{0.55\textwidth}
    
    \begin{algorithm}[H]
        \caption{Overlook this section please}
        \lblalg{softmax_top_p}
        \definecolor{codeblue}{rgb}{0.25,0.65,0.5}
        \definecolor{codeblue2}{rgb}{0,0,1}
        \lstset{
          backgroundcolor=\color{white},
          basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
          columns=fixed,
          breaklines=true,
          captionpos=b,
          commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
          keywordstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue2},
        }
        \begin{lstlisting}[language=python]
        def weighted_softmax(scores, weight):
            exp_score = torch.exp(scores)
            weighted_exp = weights * exp_score
            softmax_out = weighted_exp / torch.sum(weighted_exp)
            return softmax_out
        
        def top_p(weights, p):
            values, indices = torch.topp(weights, p, dim=-1)
            return indices
            
        \end{lstlisting}
    \end{algorithm}
    
    \end{minipage}
    
\end{figure}

==> figure_texts/ablation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Ablation.pdf}
    \caption{Ablation and sensitivity test.}
    \label{fig:ablation}
\end{figure}

==> text/1000_Checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our claims are empirically verified by \sects{experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the applicability limitation in \sects{conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the theoretical proof for the correctness of semantic permutation in \sects{methodology-permutation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All experiment details are included in \sects{experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the algorithms and implementation details are mentioned in \sects{methodology} and \sects{experiments}. Our code and scripts will be released upon publication.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All experiment hyperparameters are included in \sects{experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We test over multiple random seeds and the results are highly deterministic and reproducible. So we don't include error bar in the figure.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments are all conducted on common NVIDIA GPUs described in \sects{experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conform with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper introduces a method to accelerate video generation models, so it does not have direct societal impact. However, the use of video generation models may have social impact, which can be amplified by this technique.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will explicitly specify the usage permission of our method with proper licenses.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper uses open-source datasets and models in \sects{experiments}. The usage respects all the original licenses. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core method development in this paper does not involve LLMs as any important, original or non-standard components.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> text/1_Introduction_v0.tex <==
\section{Introduction}
\lblsect{intro}

% Video generation using diffusion models has seen remarkable progress, driven by advances in spatiotemporal transformer architectures. Recent models such as Wan 2.1~\cite{wan2025} and HunyuanVideo~\cite{kong2024hunyuanvideo} have demonstrated the capacity of diffusion transformers (DiTs) to synthesize high-quality, coherent videos across diverse prompts. Despite these advances, the computational cost associated with full 3D attention over spatial-temporal tokens remains a major bottleneck for scalable and efficient video generation.

% To address this, prior work has focused on reducing attention redundancy by exploiting architectural or data-driven sparsity. Sparse VideoGen~\cite{xi2025sparse} introduces a dynamic head specialization approach to decouple spatial and temporal attention patterns, thereby pruning redundant attention paths.

% In this paper, we propose \method, a novel framework that reduces computational redundancy in video diffusion transformers through token clustering and selective attention routing. Our approach combines two core ideas:

% 1. Token Rearrangement via K-Means Clustering: We dynamically cluster tokens in the latent space using a lightweight k-means module. Tokens within the same cluster are rearranged to form semantically coherent groups, allowing the model to process regions with similar content jointly.

% 2. Top-P Sparse Attention: Building on this structure, we introduce a top-p attention mechanism that restricts each token’s attention to only the most informative peers within or across clusters, based on content relevance. This probabilistic filtering reduces the attention matrix density without fixed spatial priors or temporal windows.

% Unlike fixed sparsity patterns or specialized attention heads, \method adapts dynamically to input content and can generalize across different video domains. It is training-free, plug-and-play, and compatible with existing DiT architectures. Additionally, we implement a hardware-efficient kernel to support our cluster-aware attention routing, achieving high memory throughput and parallelism.

% Extensive experiments on the HunyuanVideo and Wan 2.1 show that \method achieves up to \fixme with. Our method pushes the frontier of efficient video synthesis and offers a new perspective on structured sparsity in diffusion models.

\yilong{intro v0: will rewrite}


Diffusion Transformers (DiTs) have demonstrated significant efficacy in generative tasks, particularly excelling in generating high-quality images and videos~\cite{kong2024hunyuanvideo,wan2025}. However, the computational efficiency of DiTs remains a major bottleneck, primarily due to the quadratic computational complexity introduced by 3D spatio-temporal attention mechanisms~\cite{xi2025sparse}. For instance, generating just a 5-second video using HunyuanVideo on an NVIDIA A100 GPU takes nearly an hour, where the 3D attention accounts for more than $80$\% of end-to-end runtime. This inefficiency severely limiting the practical deployment of DiT-based generative models. \fixme{Potential figure}


To mitigate the quadratic computational complexity, previous studies have observed that self-attention mechanisms are naturally sparse, where only a small portion of computations significantly influence the final output~\cite{tang2024quest,zhang2023h2oheavyhitteroracleefficient,xiaoefficient}. For example, SVG~\cite{xi2025sparse} and STA~\cite{zhang2025fast} first identify sparse patterns \textit{statically} during offline. At runtime, each attention operation is then classified into one of these predefined patterns, computing attention scores only for the selected \textit{critical tokens}. This strategy reduces computational costs by up to $8\times$ with acceptable degradation in generation quality.


Recent studies have extended sparse attention from static patterns to \textit{dynamically} determined sparse patterns, achieving a better trade-off between quality and efficiency~\cite{zhang2025spargeattn, xu2025xattention}. As generative tasks are inherently diverse, attention patterns are varied during runtime~\cite{tang2024quest}. Consequently, static patterns fail to accommodate this variability, significantly reducing quality. To capture these diverse patterns, these dynamic approaches introduce an extra \textit{identification step}. During this step, runtime information from each token is used to estimate attention scores, selecting tokens with the highest scores as critical tokens. To minimize overhead, the identification is typically process at the \textit{block granularity}, treating consecutive tokens as an aggregated token, which are selected or ignored as a whole~\cite{zhu2025tacticadaptivesparseattention}.


However, we observe that given the same computational budget, existing dynamic sparse attention methods significantly fall behind the oracle attention recall, where all attention scores are known beforehand, as illustrated in Figure~\fixme{}. This performance gap arises from two primary factors.


First, current block-grained identification methods are ineffective in accurately identifying critical tokens. Because tokens are grouped into blocks based on positions rather than \textit{semantic similarities}, tokens within the same block may have dramatically different activations in the latent space. Consequently, the aggregated activations become less representative~\cite{zhu2025tacticadaptivesparseattention}, leading to inaccurate estimations of attention scores and thus incorrect selection of critical tokens. Second, even if critical tokens could be perfectly identified, current methods still suffer from inefficiencies due to the mismatch between sparse computation and hardware specifications~\cite{zheng2023pitoptimizationdynamicsparse}. Modern ML accelerators are equipped with ASIC optimized for dense general matrix multiplication (GEMM) operations that follow a fixed layout~\cite{ye2023sparsetircomposableabstractionssparse}. For instance, tensor cores on NVIDIA GPUs require a minimum GEMM size of $16\times16\times8$~\cite{a100}. Thus, even if only a subset of tokens within a block of $16$ tokens are critical, the entire block must still be computed to utilize tensor cores, causing computational waste.


To bridge this performance gap, we propose \method{}, a training-free sparse attention approach specifically designed to accelerate video generation for DiT-based models, achieving a Pareto frontier trade-off between generation quality and computational efficiency. Our key insight is to leverage \textit{\sap{}} to maximize both the accuracy of sparse pattern identification and hardware utilization during sparse computations. Specifically, \sap{} clusters tokens into blocks according to the semantic of activations rather than positions. Consequently, tokens within each block exhibit closely aligned embeddings, ensuring more accurate aggregated representations and thereby significantly improving identification accuracy. Additionally, \sap{} \textit{densifies} sparse computations by consolidating scattered critical tokens into compact, dense blocks. Due to their semantic similarity, tokens in a single block tend to be either all critical or all non-critical, substantially reducing computation waste.


To integrate \sap{} into an end-to-end framework, \method{} introduces three key designs. First, to implement \sap{}, \method{} applies \kmeans{} clustering on the Query, Key, and Value vectors of each head and layer before the identification step. The resulting clusters are then permuted so that consecutive tokens within the same cluster are grouped together, ensuring semantically coherent blocks. Second, to allow flexible computational budget rather than a fixed value, \method{} adopts a Top-p critical token selection strategy inspired by~\cite{zhu2025tacticadaptivesparseattention,lin2025twilightadaptiveattentionsparsity}. Specifically, \method{} uses the centroids of clusters to approximate attention scores for each cluster, selecting tokens with the highest scores until their cumulative sum reaches $p$. This approach enables dynamic budget allocation without manual adjustments. Finally, \method{} introduces a custom kernel implementation that supports dynamic block sizes for sparse attention. This is essential because the clusters formed by \sap{} naturally vary in size, and existing block sparse attention methods, which are limited to fixed block sizes, cannot efficiently handle such variability.


We prototype \method{} based on an open-sourced video generation framework~\cite{xi2025sparse} and customize kernels with FlashInfer~\cite{ye2025flashinferefficientcustomizableattention}. We evaluate \method{}'s quality and efficiency on representative video generative models including CogVideoX-v1.5-I2V, \fixme{}, and \fixme{}. Results demonstrate that \method{} consistently achieves a Pareto frontier, delivering superior generation quality at any given computational budget. Specifically, \method{} delivers significant efficiency improvements, achieving an end-to-end speedup of up to \fixme{} while maintaining high visual quality with a PSNR of up to \fixme{}, outperforming all prior methods.

==> text/3_Motivation_v0.tex <==
\section{Motivation}
\lblsect{motivation}
\input{figure_texts/contextual_similarity}

\subsection{Inherent Sparsity in Video DiT Attention}

Attention in video DiTs naturally exhibits a high degree of sparsity that varies dynamically.
For instance, prior work such as SVG has identified distinct spatial and temporal attention heads, which often concentrate their effective computation on a relatively small fraction—around 25-30\%—of all possible token interactions, yet these focused interactions are vital for model performance. 
This observation underscores that significant portions of the attention matrix are often sparsely populated.

To establish the upper bound for ideal sparse attention in \fixme{}, we define an oracle \topp attention: for each query, attention is computed only with the minimal subset of keys that collectively capture 90\% of its total pre-calculated attention scores. 
Our analysis demonstrates that this oracle \topp attention achieves an excellent PSNR of \fixme{} while demanding merely \fixme{e.g., 20\%} of the computational load inherent in full attention. 
Such near-lossless quality at a significantly reduced computational cost presents a vast, untapped opportunity, as current sparse attention techniques fall considerably short of this efficacy. This disparity critically motivates the development of more advanced and effective sparsity strategies.



\subsection{Limitations of Existing Video Sparse Attention}

Current approaches to sparse attention in video models, while varied, exhibit fundamental limitations when benchmarked against this oracle potential.
Static approaches, such as calibration-based methods~\citep{} and pattern-selection methods~\citep{}, which apply predefined sparse patterns, inherently struggle with the dynamic nature of video. 
As identified by SVG, video attention maps are not only sparse but also highly variable, changing with input content, across different model layers, attention heads, and even through denoising timesteps. 
The inflexibility of static or fixed patterns makes it difficult to adapt to these complex dynamics, resulting in a significant performance gap when compared to the oracle sparse attention, and often leading to suboptimal utilization of the computational budget.

% As identified by works like SVG, relevant attention patterns (e.g., spatial vs. temporal) can differ substantially not only across different layers and attention heads but also fluctuate based on the input content and even the specific denoising timestep. 
% This dynamism makes calibration-based methods fundamentally ill-suited, as their static or pre-determined biases cannot adapt to such fluid interaction landscapes. 
% Similarly, while pattern-based selection methods like SVG capture common interaction motifs, their fixed patterns may not always align with the most salient interactions for a given context.
% That is because the required computation differs even for the same attention pattern.
% Recognizing the need for adaptability, \bsa methods have incorporated dynamic computation control, often employing \topp sampling or thresholding to vary the computational budget based on input characteristics.
% Nevertheless, the performance of these block sparse techniques often remains comparable to pattern-based methods like SVG~\citep{}, failing to unlock substantial new gains. This limitation stems from two primary deficiencies:\fixme{Maybe remove itemization}

Recognizing the need for adaptability, \bsa has emerged as a promising direction, primarily because block-wise operations are amenable to modern hardware like TensorCores, facilitating high throughput and relatively low management overhead. 
Methods such as Sparge~\citep{} and XAttention~\citep{} have even incorporated dynamic computation control, often using top-p sampling to adjust the compute budget.
Nevertheless, the performance of these block sparse techniques only remains comparable to pattern-based methods like SVG~\citep{}, failing to unlock substantial new gains. This limitation stems from two primary deficiencies.

\textbf{Coarse-Grained Block Identification Misses Critical Tokens.}
Current \bsa methods typically employ approximate strategies to estimate the importance of each block before computation, aiming for efficiency. 
For instance, methods like Sparge~\citep{} utilize mean pooling, where a single representation might be derived from every 128 query tokens to interact with representations derived from every 64 key tokens. 
Such highly coarse estimations, however, often fail to accurately capture the true importance of blocks, especially when token representations within these large receptive fields are heterogeneous. 
\Andy{[Optional] While Sparge also introduces intra-block similarity refinements in an attempt to mitigate these estimation errors, this acts more as a corrective heuristic rather than addressing the fundamental inaccuracy of the initial coarse block assessment.} 
Consequently, as our analyses in Section~\ref{} demonstrate, this inherent imprecision in block importance estimation leads to a significant \textit{Critical Block Miss Rate}, where blocks containing tokens with genuinely high attention scores are erroneously discarded.


\textbf{Heterogeneity within Selected Blocks Causes Significant Computational Waste.}
A more fundamental issue persists even if a block containing some important tokens is correctly selected. 
If the tokens within this block exhibit diverse attention scores—mixing high-importance interactions with many low-importance ones, a large fraction of the computation performed on that block is effectively wasted. 
For example, the temporal attention heads in SVG~\citep{} exhibit highly scattered attention patterns, where individual tokens with high attention scores are interspersed with many low-scoring neighbors. 
When \bsa is applied, any block selected to cover these critical scattered tokens will inevitably also encompass numerous unnecessary low-score tokens, leading to inefficient computation within the chosen block. 
Our quantitative evaluations in Section~\ref{} reveal that for existing \bsa methods, the proportion of computation spent on non-critical token pairs within selected blocks can be notably high. 
This means a large portion of the theoretical FLOPs reduction is consumed by processing token pairs that contribute minimally to the attention output, preventing these savings from fully translating into commensurate end-to-end speedups.


% \textbf{Coarse-Grained Block Identification Misses Critical Tokens.}
% Current \bsa methods typically employ approximate strategies (e.g., feature pooling or sampling within predefined blocks) to estimate the importance of each block before selection.
% \fixme{Add sparge as an example. Use mean pooling. Every 128 queries use one representation and every 64 keys use one representation}
% These coarse estimations often fail to accurately capture the true importance of blocks, especially when token representations within them are heterogeneous. 
% \fixme{Add example: Sparge attempt to mitigate this by introducing intra-block similarity refinements (e.g., cosine similarity)}
% As our analyses in Section~\ref{} demonstrate, this inaccuracy leads to a significant \textit{Critical Block Miss Rate}, where blocks containing tokens with high attention scores are discarded. 

% \textbf{Heterogeneity within Selected Blocks Causes Significant Computational Waste.}
% A more fundamental issue persists even if a block containing important tokens is correctly selected. 
% If the tokens within this block exhibit diverse attention scores—mixing high-importance interactions with many low-importance ones—a large fraction of the computation performed on that block is effectively wasted.
% \fixme{Add example: The temporal head in SVG shows that tokens with high attention scores might be really scattered. block sparse attention will inevitably compute those unnecessary blocks.}
% Our quantitative evaluations in Section~\ref{} reveal that for existing \bsa methods, the \fixme{computation needed with oracle block selection} can be notably high. 
% This means a large portion of FLOPS is spent on token pairs that contribute little, preventing the theoretical FLOPs reduction from translating into commensurate end-to-end speedups.

% \begin{itemize}
%     \item \textbf{Inaccurate block importance estimation.} To efficiently select which blocks to compute, current block sparse methods typically rely on coarse approximations of block importance, such as mean pooling or sampling. 
%     Such approximations can be highly inaccurate, especially when token representations within a block exhibit high variance. While some methods like Sparge attempt to mitigate this by introducing intra-block similarity refinements (e.g., cosine similarity), these often act as heuristics that do not fundamentally resolve the inaccuracy of the initial estimation.
%     \item \textbf{Inefficient computation within selected blocks.} A more critical issue persists even if blocks could be selected with oracle estimation. If a selected block contains a mix of tokens with high attention scores alongside tokens with low attention scores, significant computational resources are squandered on computing interactions involving these low-importance tokens. 
%     This is particularly problematic in scenarios with scattered attention pattern, such as the temporal head attention illustrated by SVG, where applying a coarse block structure over such patterns inevitably leads to substantial inefficient computation.
% \end{itemize}


% \subsection{Our Approach: Dynamic Grouping for Efficient Sparse Attention}

% In this work, we propose a novel approach to video sparse attention that directly addresses the aforementioned challenges. 
% \fixme{Add reference for layout transformation in temporal head?} The core intuition is simple yet powerful: dynamically group semantically similar tokens together before computing attention. 
% By leveraging techniques such as \kmeans clustering on query and key tokens, we re-organize tokens such that those with similar semantic features are contiguous for computation.
% This "cluster-then-compute" strategy offers a direct solution to the two primary deficiencies identified in existing block sparse methods.

% \textbf{Enhanced Accuracy in Block Importance Estimation.} By clustering tokens first, the variance of token representations within each resulting group (cluster) is inherently reduced compared to arbitrary or spatially fixed blocks. 
% Consequently, using the centroid of a cluster as its representative feature provides a much more accurate basis for estimating inter-block attention scores.

% \textbf{Improved Computational Efficiency.} Since tokens within a cluster are semantically similar, their attention responses to other tokens are also more likely to be homogeneous. 
% When attention blocks are formed based on these clusters and selected, the chosen blocks will predominantly contain tokens of similar importance.
% This significantly reduces the issue of high- and low-attention tokens being intermingled, leading to a more effective application of the computational budget on genuinely important interactions.


% \subsection{Limitations of Static Sparse Attention}

% Video data exhibits rich spatial and temporal coherence, with many regions remaining static or semantically similar across frames. Transformer-based video diffusion models, however, often treat all token interactions equally, resulting in inefficient attention computation.

% Prior sparse attention strategies—such as block-sparse attention or fixed temporal heads—rely on static patterns that do not adapt to content. For example, block-sparse attention uses fixed regions, which can easily miss meaningful long-range or dynamic interactions. Similarly, top-$k$ attention retains the top $k$ attention scores regardless of how attention is distributed, enforcing a rigid threshold that may ignore important but less dominant signals.

% However, attention distributions in video diffusion are highly non-uniform and dynamic. The optimal sparsity varies across layers, attention heads, and time steps. This makes any fixed-pattern approach fundamentally inadequate.

% To handle this variability, a dynamic sparsification method is needed—one that allocates attention computation based on the actual distribution of relevance in each context.




% \subsection{Inefficiency of Naive Dynamic Attention and the Role of Contextual Similarity}
% % \input{figure_texts/contextual_similarity}

% While dynamic strategies such as top-$p$ attention offer flexibility by retaining a variable number of tokens based on cumulative attention mass, they can still lead to inefficient computation if large attention scores are scattered throughout the map. Even when attention is selectively computed, high scores that are spread across distant or unrelated regions still require computing many unimportant token interactions.

% This inefficiency is due to how attention maps are structured. Because attention is permutation-invariant, we are free to reorder tokens. If similar tokens—such as spatially or semantically coherent regions—are grouped together, the large attention scores can be concentrated into tighter regions. This spatial locality enables more efficient attention computation, avoiding waste from sparsely scattered high scores.

% Existing approaches like Temporal Head take steps in this direction by grouping tokens temporally, but their design is too simplistic and static to fully exploit the potential efficiency gains.


% \subsection{Inefficiency of Current Attention Mechanisms}

% Video data exhibits strong spatial and temporal coherence, often characterized by regions that change minimally across frames or share similar semantic content. In video diffusion models, this coherence manifests as a high degree of contextual similarity among tokens.

% This contextual redundancy results in highly repetitive patterns within the full attention maps generated by transformer-based architectures. Rather than treating all token interactions uniformly, this observation suggests that a more efficient approach would involve grouping tokens that are semantically and contextually similar. By identifying and clustering these similar tokens, the model can perform selective attention computations focused on informative or dynamic regions, thereby reducing unnecessary overhead.


% \subsection{Limitations of Static and Fixed-Pattern Sparse Attention}
% We find that attention map's optimal density pattern in highly non-static. Optimal sparsity differs every head, and patterns are also non-static. This makes previous fixed pattern works suck as sparse video gen less effective.

% Top-k attention has been proposed as a sparse attention strategy by preserving only the highest attention weights. However, it imposes a hard constraint on the number of attended tokens, regardless of their actual distribution. In contrast, top-p attention considers a variable number of tokens that cumulatively account for a predefined proportion $p$ of the attention scores. This leads to more flexible and context-aware sparsification, especially beneficial when the distribution of attention weights is skewed.


% \subsection{Attention is permutation invariant}
% We find that the attention mechanism is invariant to permutation on query, key, and value tensors, as long as we apply the same permutation to key and value. No restriction for query tensor.

% The scaled dot-product attention mechanism is defined as:
% \[
% \text{Attention}(Q, K, V) = \text{softmax}\left(\frac{QK^\top}{\sqrt{d_k}}\right)V
% \]
% where \( Q \in \mathbb{R}^{n \times d_k} \), \( K, V \in \mathbb{R}^{m \times d_k} \) and \( \mathbb{R}^{m \times d_v} \), and \( d_k \) is the key/query dimensionality.

% Let \( P_1 \in \mathbb{R}^{n \times n} \) and \( P_2 \in \mathbb{R}^{m \times m} \) be permutation matrices, where $P_1 P_1^T = I, P_2 P_2^T = I$. Define the permuted inputs:
% \[
% \tilde{Q} = P_1 Q, \quad \tilde{K} = P_2 K, \quad \tilde{V} = P_2 V.
% \]

% Then the attention output under these permutations is:
% \begin{align}
% & P_1^\top \text{Attention}(\tilde{Q}, \tilde{K}, \tilde{V}) 
% = P_1^\top \text{softmax}\left( \frac{P_1 Q K^\top P_2^\top}{\sqrt{d_k}} \right) P_2 V \\
% =& P_1^\top P_1 \text{softmax}\left( \frac{Q K^\top}{\sqrt{d_k}} \right) P_2^\top P_2 V
% = \text{softmax}\left( \frac{Q K^\top}{\sqrt{d_k}} \right) V
% \end{align}

% Thus, applying known permutations to \( Q \), \( K \), and \( V \) can be inverted or undone to recover the original attention output.


% \input{figure_texts/highlevel_idea}

